Talk More Listen Less: Energy-Efficient Neighbor Discovery in Wireless Sensor Networks

Neighbor discovery is a fundamental service for initialization and managing network dynamics in wireless sensor networks and mobile sensing applications. In this paper, we present a novel design principle named Talk More Listen Less (TMLL) to reduce idle-listening in neighbor discovery protocols by learning the fact that more beacons lead to fewer wakeups. We propose an extended neighbor discovery model for analyzing wakeup schedules in which beacons are not necessarily placed in the wakeup slots. Furthermore, we are the first to consider channel occupancy rate in discovery protocols by introducing a new metric to trade off among duty-cycle, latency and channel occupancy rate. Guided by the TMLL principle, we have designed Nihao, a family of energy-efficient asynchronous neighbor discovery protocols for symmetric and asymmetric cases. We compared Nihao with existing state of the art protocols via analysis and real-world testbed experiments. The result shows that Nihao significantly outperforms the others both in theory and practice.

==> Makefile <==
LATEX=pdflatex
default:
	$(LATEX) main.tex
	$(LATEX) main.tex

all:
	$(LATEX) main.tex
	bibtex  main
	$(LATEX) main.tex
	$(LATEX) main.tex
	pdftops main.pdf
	ps2pdf14 -dPDFSETTINGS=/prepress main.ps

clean:
	find -name "*.aux" -exec rm -v {} \;
	find -name "*.blg" -exec rm -v {} \;
	find -name "*.thm" -exec rm -v {} \;
	find -name "*.log" -exec rm -v {} \;
	find -name "*.out" -exec rm -v {} \;
	find -name "*.toc" -exec rm -v {} \;
	find -name "*.bbl" -exec rm -v {} \;

